Incremental Learning Techniques for Semantic Segmentation

Deep learning architectures exhibit a critical drop of performance due to catastrophic forgetting when they are required to incrementally learn new tasks. Contemporary incremental learning frameworks focus on image classification and object detection while in this work we formally introduce the incremental learning problem for semantic segmentation in which a pixel-wise labeling is considered. To tackle this task we propose to distill the knowledge of the previous model to retain the information about previously learned classes, whilst updating the current model to learn the new ones. We propose various approaches working both on the output logits and on intermediate features. In opposition to some recent frameworks, we do not store any image from previously learned classes and only the last model is needed to preserve high accuracy on these classes. The experimental evaluation on the Pascal VOC2012 dataset shows the effectiveness of the proposed approaches.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

%% All related tasks: continual learning, lifelong learning, transfer learning, multi-task learning
The incremental learning %is strictly related to other task definitions such as continual learning, lifelong learning, transfer learning, multi-task learning and never ending learning. All these 
problem require to design an algorithm that it is able to learn new tasks over time without forgetting the previously learned ones.
%% catastrophic forgetting
Indeed, deep convolutional neural networks suffer from \textit{catastrophic forgetting} \cite{mccloskey1989catastrophic, french1999catastrophic, goodfellow2013empirical} when learning new tasks. This phenomenon, which still represents one of the main limitations of neural networks, %Human brain, on the other hand, can efficiently learn new tasks and it turns out that this ability is essential for the deployment of artificial intelligence systems in challenging scenarios where new tasks or classes appear over time. 
it has been addressed even before the rise of neural networks popularity \cite{thrun1996learning, polikar2001learn, cauwenberghs2001incremental} and more recently has been rediscovered and tackled in different ways. 

Some methods \cite{xiao2014error, roy2018tree} exploit network architectures which grow over time as a tree structure in a hierarchical manner as new classes are observed. 
Istrate et al. \cite{istrate2018incremental} proposed a method that partitions the original network into sub-networks which are then gradually incorporated in the main network during the training process.
In \cite{sarwar2017incremental} the network incrementally grows over time while sharing portions of the base network.

Alternatively, a different strategy consists in freezing or slowing down the learning process in some parts of the network.
Kirkpatrick et al. \cite{kirkpatrick2017overcoming} developed Elastic Weight Consolidation (EWC) to remember old tasks by slowing down the learning process on the weights important for those tasks. In \cite{oquab2014learning} the authors identified that it is possible to minimize forgetting by freezing the earlier and the mid-level layers of the models. A similar idea has been employed in recent studies, such as \cite{li2018learning, istrate2018incremental}.


%%% distillation
Another way of retaining high performance on old tasks which has recently gained wide success is knowledge distillation. This technique was originally proposed in \cite{hinton2015distilling, bucilua2006model} to preserve the output of a complex ensemble of networks when adopting a simpler network for more efficient deployment. This idea was  adapted in different ways in recent studies \cite{shmelkov2017incremental, rebuffi2017icarl, li2018learning, wu2018incremental, castro2018end, zhou2019M2KD, furlanello2016active} to maintain the responses of the network on the old tasks whilst updating it with new training samples. We investigated this concept and we further adapted it to the semantic segmentation task, while previous works focused on object detection or classification problems.



% papers that use old data
As regards object detection and classification problems, some studies keep a small portion of data belonging to previous tasks and use them to preserve the accuracy on old tasks when dealing with new problems \cite{rebuffi2017icarl, lopez2017gradient, chaudhry2018riemannian, hou2018lifelong, castro2018end, tasar2018incremental}. In those works the exemplar set to store is chosen according to different criteria. % da riscrivere meglio
In \cite{rebuffi2017icarl, lopez2017gradient} the authors use an episodic memory which stores a subset of the observed examples from previous tasks, while incrementally learning new classes.
In \cite{chaudhry2018riemannian} a fraction of previous classes is kept as a way to alleviate intransigence of a model, i.e. the inability of a model to update its knowledge. 
Hou et al. \cite{hou2018lifelong} tried to balance between preservation and adaptation of the model via distillation and retrospection by caching a small subset of randomly picked data for old tasks.
In \cite{castro2018end} the classifier and the features for selecting the samples to be added in the representative memory are learned jointly, in an end-to-end fashion, and herding selection is used to select them.
In \cite{tasar2018incremental} the authors store some patches chosen according to an importance value determined by a weight assigned to each class and some other patches chosen at random.
However, storing previously seen data could represent a serious limitation for certain applications where privacy issues or limited storage budgets are present: indeed, selecting and storing exemplars is not scalable.
Another example of this family is the only work on incremental learning for semantic segmentation  \cite{tasar2018incremental}, which however  focused on a very specific setting related to satellite images and has several limitations when applied to generic semantic segmentation problems. Indeed, it considers the segmentation task as a multi-task learning problem, where  a binary classification for each class replaces the multi-class labeling. %Their output is then a three dimensional matrix that is a stack of binary predicted maps for all the classes. They used it for a maximum of ten classes and applied to satellite datasets. 
 Furthermore they assumed that the training images corresponding to an incremental step only contain the new classes and the capabilities on the old ones are preserved by storing a subset of the old images.
However, for large amount of classes and more various range of application the methodology does not scale properly. %These, however, are not valid assumptions for semantic segmentation problems where it is not possible to store previous images or new and old classes coexist in the scene. \textbf{[CHECK CORRECTNESS]}

% papers who don't use old data and use GANs
For this reason, some recent methods \cite{wu2018incremental, shin2017continual}, instead, do not store old data but compensate this by training Generative Adversarial Networks (GANs) to generate images containing previous classes when new classes should be learned, thus retaining high accuracy on old tasks.

% papers who don't use old data
Additionally, some other approaches, do not make use of exemplars set at all \cite{shmelkov2017incremental, kirkpatrick2017overcoming, li2018learning, dhar2018learning, aljundi2018memory, zhou2019M2KD}. 
In \cite{shmelkov2017incremental} an end-to-end learning framework is proposed where the representation and the classifier are learned jointly without storing any of the original training samples.
In \cite{li2018learning} previous knowledge is distilled directly from the last trained model. 
Dhar et al. \cite{dhar2018learning} introduced an attention distillation loss as an information preserving penalty for the classifiers' attention maps. 
Aljundi et al. \cite{aljundi2018memory} introduced the idea that when learning a new task, changes to important parameters can be penalized, effectively preventing meaningful knowledge related to previous tasks from being overwritten. 
In \cite{zhou2019M2KD} the current model distills the knowledge from all previous model snapshots, of which a pruned version is saved for memory efficiency.


Our aim is then to propose a more general framework where we do not store any previous image and the new training dataset contains also previously learned classes, thus it can be exploited to overcome their catastrophic forgetting. To the best of our knowledge this is the first study on incremental learning for semantic segmentation which does not retain previously seen images and it evaluates on standard datasets, like Pascal VOC2012 \cite{pascalvoc2012}.

